Molly: A Verified Compiler for Cryptoprotocol Roles

Molly is a program that compiles cryptographic protocol roles written in a high-level notation into straight-line programs in an intermediate-level imperative language, suitable for implementation in a conventional programming language. We define a denotational semantics for protocol roles based on an axiomatization of the runtime. A notable feature of our approach is that we assume that encryption is randomized. Thus, at the runtime level we treat encryption as a relation rather than a function. Molly is written in Coq, and generates a machine-checked proof that the procedure it constructs is correct with respect to the runtime semantics. Using Coq's extraction mechanism, one can build an efficient functional program for compilation.

==> cleantex <==
#!/bin/bash

# remove auxilliary files generated by TeX and AucTeX

find . \( -name "*~" -o -name "*.aux" -o -name "*.log" -o -name "*.lof" -o -name "*.loy" -o -name "*.toc" -o -name "*.bbl" -o -name "*.tmp" -o -name "*.bak" -o -name "*.xyc" -o -name "*.dvi" -o -name "*.out"   -o -name "*.fls" -o -name "*.fdb_latexmk" -o -name "*.blg" -o -name "*.pdfsync" -o -name "*.gz" -o -name "*.fls" -o -name "*.rel" -o -name "*.nav" -o -name "*.snm" -o -name "*.vrb" -o -name "*.rip"  -o -name "*.cb"  -o -name "*.cb2" \) -print0 | xargs -0 rm

# find . \( -name "*~" \) -print0 | xargs -0 rm 


find . -name 'auto' -print | xargs rm -rf

